Navigates Like Me: Understanding How People Evaluate Human-Like AI in Video Games

We aim to understand how people assess human likeness in navigation produced by people and artificially intelligent (AI) agents in a video game. To this end, we propose a novel AI agent with the goal of generating more human-like behavior. We collect hundreds of crowd-sourced assessments comparing the human-likeness of navigation behavior generated by our agent and baseline AI agents with human-generated behavior. Our proposed agent passes a Turing Test, while the baseline agents do not. By passing a Turing Test, we mean that human judges could not quantitatively distinguish between videos of a person and an AI agent navigating. To understand what people believe constitutes human-like navigation, we extensively analyze the justifications of these assessments. This work provides insights into the characteristics that people consider human-like in the context of goal-directed video game navigation, which is a key step for further improving human interactions with AI agents.

==> sections/00-commands_notation.tex <==
% custom commands
\newcommand{\todo}[1]{\textcolor{red}{#1}}
\newcommand{\smnote}[1]{\textcolor{black}{#1}}
\newcommand{\smchange}[1]{\textcolor{orange}{#1}}
\newcommand{\rgchange}[1]{\textcolor{blue}}
\newcommand{\uk}{United Kingdom}
\newcommand{\cam}{Cambridge}
\newcommand{\appx}{Supplemental Research Methods}
\newcommand{\rs}{reward-shaping}
\newcommand{\studyone}{\textit{hybrid} agent}
\newcommand{\studytwo}{\textit{symbolic} agent}
\newcommand{\studythree}{\emph{\rs} agent}
\newcommand{\numagreement}{$53$}
\newcommand{\rulesep}{\unskip\ \vrule\ }
\newcommand{\numtotalhntt}{6}

\definecolor{bluehl}{rgb}{0.8706,.921568,.9686274} 
\definecolor{purplehl}{rgb}{0.88627,0.815686,0.941176} 
\definecolor{orangehl}{rgb}{0.9843,0.898,0.83922} 
